On the Challenges of Open World Recognitionunder Shifting Visual Domains

Robotic visual systems operating in the wild must act in unconstrained scenarios, under different environmental conditions while facing a variety of semantic concepts, including unknown ones. To this end, recent works tried to empower visual object recognition methods with the capability to i) detect unseen concepts and ii) extended their knowledge over time, as images of new semantic classes arrive. This setting, called Open World Recognition (OWR), has the goal to produce systems capable of breaking the semantic limits present in the initial training set. However, this training set imposes to the system not only its own semantic limits, but also environmental ones, due to its bias toward certain acquisition conditions that do not necessarily reflect the high variability of the real-world. This discrepancy between training and test distribution is called domain-shift. This work investigates whether OWR algorithms are effective under domain-shift, presenting the first benchmark setup for assessing fairly the performances of OWR algorithms, with and without domain-shift. We then use this benchmark to conduct analyses in various scenarios, showing how existing OWR algorithms indeed suffer a severe performance degradation when train and test distributions differ. Our analysis shows that this degradation is only slightly mitigated by coupling OWR with domain generalization techniques, indicating that the mere plug-and-play of existing algorithms is not enough to recognize new and unknown categories in unseen domains. Our results clearly point toward open issues and future research directions, that need to be investigated for building robot visual systems able to function reliably under these challenging yet very real conditions. Code available at https://github.com/DarioFontanel/OWR-VisualDomains

==> sections/tables.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
%  & \multicolumn{4}{c|}{CW without rejection} &  \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} &  \\ \hline
% METHOD & 11 & 16 & 21 & 26 & \multicolumn{1}{c|}{Avg.} \\ \hline
% NNO & 28.8 & 19.2 & 14.2 & 11.4 & 18.4 \\ \hline
%  &  &  &  &  &  \\ \hline
% DeepNNO & 28.1 & 20.5 & 18.6 & 17.8 & 21.3 \\ \hline
% DeepNNO-RDA & 43.0 & 36.3 & 29.4 & 25.6 & 33.6 \\ \hline
% DeepNNO-RSDA & 41.4 & 35.9 & 29.9 & 25.8 & 33.3 \\ \hline
% DeepNNO-rot & 27.1 & 19.5 & 16.9 & 17.0 & 20.1 \\ \hline
% DeepNNO-RDA-rot & 43.4 & 35.0 & 29.9 & 25.9 & 33.5 \\ \hline
% DeepNNO-Dropout & 27.9 & 21.0 & 19.9 & 19.0 & 21.9 \\ \hline
%  &  &  &  &  &  \\ \hline
% B-DOC & 27.8 & 21.0 & 20.2 & 20.0 & 22.3 \\ \hline
% B-DOC-RDA & 44.6 & 37.8 & 29.0 & 22.6 & 33.5 \\ \hline
% B-DOC-RSDA & 43.0 & 34.7 & 26.1 & 23.7 & 31.9 \\ \hline
% B-DOC-rot & 28.5 & 19.8 & 18.8 & 18.7 & 21.4 \\ \hline
% B-DOC-RDA-rot & 43.1 & 35.7 & 27.7 & 22.6 & 32.2 \\ \hline
% \end{tabular}
% \caption{Closed World Without Rejection ROD - ARID%\vspace{-20pt}
% }
% \label{tab:cw_without_rod_arid}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|c|}
% \hline
%  & \multicolumn{4}{c|}{CW with rejection} & \multicolumn{1}{l|}{} \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{} \\ \hline
% METHOD & 11 & 16 & 21 & 26 & Avg. \\ \hline
% NNO & 3.5 & 3.2 & 2.9 & 2.7 & 3.1 \\ \hline
%  &  &  &  &  &  \\ \hline
% DeepNNO & 4.4 & 7.7 & 8.1 & 9.1 & 7.3 \\ \hline
% DeepNNO-RDA & 12.5 & 22.3 & 19.2 & 15.4 & 17.4 \\ \hline
% DeepNNO-RSDA & 12.8 & 16.9 & 15.4 & 14.4 & 14.9 \\ \hline
% DeepNNO-rot & 3.6 & 6.5 & 6.6 & 8.3 & 6.3 \\ \hline
% DeepNNO-RDA-rot & 12.7 & 18.8 & 17.3 & 15.3 & 16.0 \\ \hline
% DeepNNO-Dropout & 12.9 & 14.3 & 14.7 & 14.2 & 14.0 \\ \hline
%  &  &  &  &  &  \\ \hline
% B-DOC & 14.9 & 10.5 & 7.5 & 6.9 & 10.0 \\ \hline
% B-DOC-RDA & 13.9 & 13.9 & 8.5 & 5.1 & 10.4 \\ \hline
% B-DOC-RSDA & 18.1 & 15.5 & 8.8 & 6.5 & 12.2 \\ \hline
% B-DOC-rot & 17.2 & 10.6 & 7.5 & 7.3 & 10.6 \\ \hline
% B-DOC-RDA-rot & 15.6 & 15.5 & 9.3 & 6.3 & 11.7 \\ \hline
% \end{tabular}
% \caption{Closed World With Rejection ROD - ARID}
% \label{tab:cw_with_rod_arid}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|c|r|}
% \hline
%  & \multicolumn{4}{c|}{Open World} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
% METHOD & 11 & 16 & 21 & 26 & Avg. & \multicolumn{1}{l|}{Harm} \\ \hline
% NNO & 49.4 & 46.3 & 44.0 & 42.3 & 45.5 & 5.9 \\ \hline
%  &  &  &  &  &  & \multicolumn{1}{l|}{} \\ \hline
% DeepNNO & 48.9 & 42.7 & 40.6 & 39.5 & 42.9 & 13.4 \\ \hline
% DeepNNO-RDA & 49.0 & 38.6 & 36.1 & 34.5 & 39.5 & 27.1 \\ \hline
% DeepNNO-RSDA & 48.5 & 44.8 & 40.6 & 37.7 & 42.9 & 24.6 \\ \hline
% DeepNNO-rot & 48.7 & 42.3 & 41.6 & 41.0 & 43.4 & 11.6 \\ \hline
% DeepNNO-RDA-rot & 49.1 & 41.9 & 38.7 & 35.5 & 41.3 & 25.8 \\ \hline
% DeepNNO-Dropout & 41.6 & 30.6 & 30.1 & 29.8 & 33.0 & 22.1 \\ \hline
%  &  &  &  &  &  & \multicolumn{1}{l|}{} \\ \hline
% B-DOC & 41.2 & 38.8 & 42.6 & 44.1 & 41.7 & 17.5 \\ \hline
% B-DOC-RDA & 49.8 & 47.9 & 46.7 & 46.3 & 47.7 & 18.5 \\ \hline
% B-DOC-RSDA & 46.8 & 44.1 & 44.5 & 45.7 & 45.2 & 21.1 \\ \hline
% B-DOC-rot & 40.0 & 38.5 & 41.6 & 43.8 & 40.9 & 18.5 \\ \hline
% B-DOC-RDA-rot & 48.9 & 46.0 & 44.9 & 44.8 & 46.1 & 20.4 \\ \hline
% \end{tabular}
% \caption{OWR mean ROD - ARID}
% \label{tab:owr_rod_arid}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|c|}
% \hline
%  & \multicolumn{4}{c|}{CW without rejection} & \multicolumn{1}{l|}{} \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{} \\ \hline
% METHOD & 11 & 16 & 21 & 26 & Avg. \\ \hline
% NNO & 79.2 & 61.6 & 52.9 & 42.5 & 59.1 \\ \hline
%  & 79.2 & 70.8 & 67.5 & 60.1 & 69.4 \\ \hline
% DeepNNO & 87.8 & 77.8 & 72.9 & 64.3 & 75.7 \\ \hline
% DeepNNO-RDA & 87.1 & 79.1 & 73.0 & 65.5 & 76.2 \\ \hline
% DeepNNO-RSDA & 79.5 & 68.8 & 64.1 & 58.1 & 67.6 \\ \hline
% DeepNNO-rot & 86.6 & 78.8 & 73.7 & 67.3 & 76.6 \\ \hline
% DeepNNO-RDA-rot & 77.4 & 67.7 & 64.0 & 58.9 & 67.0 \\ \hline
% DeepNNO-Dropout & 80.6 & 69.9 & 66.7 & 57.9 & 68.8 \\ \hline
%  & 89.8 & 77.2 & 71.8 & 64.8 & 75.9 \\ \hline
% B-DOC & 86.4 & 76.6 & 69.0 & 61.9 & 73.5 \\ \hline
% B-DOC-RDA & 80.9 & 71.5 & 67.5 & 60.7 & 70.2 \\ \hline
% B-DOC-RSDA & 90.9 & 77.3 & 68.7 & 62.8 & 74.9 \\ \hline
% B-DOC-rot & 40.0 & 38.5 & 41.6 & 43.8 & 40.9 \\ \hline
% B-DOC-RDA-rot & 48.9 & 46.0 & 44.9 & 44.8 & 46.1 \\ \hline
% \end{tabular}
% \caption{Closed World Without Rejection ROD - ROD}
% \label{tab:cw_without_rod_rod}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|c|}
% \hline
%  & \multicolumn{4}{c|}{CW with rejection} & \multicolumn{1}{l|}{} \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{} \\ \hline
% METHOD & 11 & 16 & 21 & 26 & Avg. \\ \hline
% NNO & 36.1 & 29.6 & 27.2 & 23.0 & 29.0 \\ \hline
%  & 43.9 & 51.6 & 53.6 & 49.6 & 49.7 \\ \hline
% DeepNNO & 55.7 & 66.3 & 64.1 & 55.9 & 60.5 \\ \hline
% DeepNNO-RDA & 55.7 & 60.8 & 61.4 & 56.3 & 58.5 \\ \hline
% DeepNNO-RSDA & 44.4 & 50.5 & 50.1 & 46.5 & 47.9 \\ \hline
% DeepNNO-rot & 54.7 & 62.7 & 63.4 & 58.9 & 59.9 \\ \hline
% DeepNNO-RDA-rot & 64.4 & 60.8 & 58.0 & 53.4 & 59.2 \\ \hline
% DeepNNO-Dropout & 70.6 & 59.5 & 53.8 & 40.3 & 56.0 \\ \hline
%  & 63.5 & 59.5 & 52.3 & 42.7 & 54.5 \\ \hline
% B-DOC & 68.0 & 61.1 & 51.8 & 42.5 & 55.9 \\ \hline
% B-DOC-RDA & 74.0 & 63.2 & 56.4 & 44.4 & 59.5 \\ \hline
% B-DOC-RSDA & 65.4 & 57.1 & 49.4 & 41.3 & 53.3 \\ \hline
% B-DOC-rot & 40.0 & 38.5 & 41.6 & 43.8 & 40.9 \\ \hline
% B-DOC-RDA-rot & 48.9 & 46.0 & 44.9 & 44.8 & 46.1 \\ \hline
% \end{tabular}
% \caption{Closed World With Rejection ROD - ROD}
% \label{tab:cw_with_rod_rod}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|c|r|}
% \hline
%  & \multicolumn{4}{c|}{Open World} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
% METHOD & 11 & 16 & 21 & 26 & Avg. & \multicolumn{1}{l|}{Harm} \\ \hline
% NNO & 63.3 & 55.4 & 50.6 & 46.0 & 53.8 & 42.3 \\ \hline
%  &  &  &  &  &  & \multicolumn{1}{l|}{} \\ \hline
% DeepNNO & 66.8 & 61.0 & 57.8 & 52.6 & 59.5 & 57.9 \\ \hline
% DeepNNO-RDA & 75.7 & 73.9 & 72.1 & 65.7 & 71.9 & 70.1 \\ \hline
% DeepNNO-RSDA & 65.3 & 58.5 & 53.6 & 49.0 & 56.6 & 56.5 \\ \hline
% DeepNNO-rot & 66.8 & 59.4 & 55.4 & 50.8 & 58.1 & 56.3 \\ \hline
% DeepNNO-RDA-rot & 66.5 & 58.4 & 52.7 & 48.6 & 56.5 & 56.3 \\ \hline
% DeepNNO-Dropout & 63.7 & 49.0 & 45.5 & 40.7 & 49.7 & 48.0 \\ \hline
%  &  &  &  &  &  & \multicolumn{1}{l|}{} \\ \hline
% B-DOC & 64.5 & 56.2 & 59.7 & 54.7 & 58.8 & 58.7 \\ \hline
% B-DOC-RDA & 68.8 & 62.3 & 60.3 & 56.1 & 61.9 & 61.0 \\ \hline
% B-DOC-RSDA & 65.0 & 58.1 & 56.7 & 54.8 & 58.6 & 58.5 \\ \hline
% B-DOC-rot & 60.9 & 55.6 & 57.8 & 54.6 & 57.2 & 57.2 \\ \hline
% B-DOC-RDA-rot & 67.6 & 58.6 & 55.7 & 53.2 & 58.8 & 58.3 \\ \hline
% \end{tabular}
% \caption{OWR mea ROD - ROD}
% \label{tab:owr_rod_rod}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|c|}
% \hline
%  & \multicolumn{4}{c|}{CW without rejection} & \multicolumn{1}{l|}{} \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{} \\ \hline
% METHOD & 11 & 16 & 21 & 26 & Avg. \\ \hline
% NNO & 11.9 & 8.0 & 6.5 & 5.3 & 7.9 \\ \hline
%  &  &  &  &  &  \\ \hline
% DeepNNO & 12.6 & 8.8 & 8.8 & 6.9 & 9.3 \\ \hline
% DeepNNO-RDA & 18.5 & 12.7 & 9.8 & 7.9 & 12.2 \\ \hline
% DeepNNO-RSDA & 17.0 & 10.9 & 8.8 & 7.0 & 10.9 \\ \hline
% DeepNNO-rot & 12.7 & 8.5 & 8.3 & 6.6 & 9.0 \\ \hline
% DeepNNO-RDA-rot & 18.6 & 11.9 & 9.0 & 7.3 & 11.7 \\ \hline
% DeepNNO-Dropout & 12.5 & 9.0 & 10.1 & 7.3 & 9.7 \\ \hline
%  &  &  &  &  &  \\ \hline
% B-DOC & 12.6 & 8.6 & 9.1 & 6.4 & 9.2 \\ \hline
% B-DOC-RDA & 19.7 & 13.7 & 10.6 & 8.3 & 13.1 \\ \hline
% B-DOC-RSDA & 18.7 & 13.4 & 10.2 & 7.7 & 12.5 \\ \hline
% B-DOC-rot & 11.6 & 8.7 & 8.8 & 6.3 & 8.8 \\ \hline
% B-DOC-RDA-rot & \multicolumn{1}{r|}{19.6} & \multicolumn{1}{r|}{13.5} & \multicolumn{1}{r|}{10.9} & \multicolumn{1}{r|}{8.0} & 13.0 \\ \hline
% \end{tabular}
% \caption{Closed World Without Rejection ROD - synROD}
% \label{tab:cw_without_rod_synrod}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|c|}
% \hline
%  & \multicolumn{4}{c|}{CW with rejection} & \multicolumn{1}{l|}{} \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{} \\ \hline
% METHOD & 11 & 16 & 21 & 26 & Avg. \\ \hline
% NNO & 0.3 & 0.4 & 0.5 & 0.6 & 0.4 \\ \hline
%  &  &  &  &  &  \\ \hline
% DeepNNO & 0.8 & 2.1 & 2.2 & 2.2 & 1.8 \\ \hline
% DeepNNO-RDA & 2.5 & 5.2 & 4.7 & 3.8 & 4.0 \\ \hline
% DeepNNO-RSDA & 2.5 & 2.7 & 2.7 & 2.9 & 2.7 \\ \hline
% DeepNNO-rot & 0.6 & 1.7 & 1.9 & 1.9 & 1.5 \\ \hline
% DeepNNO-RDA-rot & 2.3 & 3.6 & 3.7 & 3.4 & 3.3 \\ \hline
% DeepNNO-Dropout & 4.4 & 4.6 & 5.8 & 4.2 & 4.7 \\ \hline
%  &  &  &  &  &  \\ \hline
% B-DOC & 3.5 & 1.8 & 1.2 & 1.0 & 1.9 \\ \hline
% B-DOC-RDA & 2.7 & 3.0 & 2.0 & 1.5 & 2.3 \\ \hline
% B-DOC-RSDA & 4.3 & 3.6 & 2.2 & 1.3 & 2.9 \\ \hline
% B-DOC-rot & 3.4 & 1.9 & 1.4 & 1.3 & 2.0 \\ \hline
% B-DOC-RDA-rot & \multicolumn{1}{r|}{3.6} & \multicolumn{1}{r|}{3.7} & \multicolumn{1}{r|}{2.5} & \multicolumn{1}{r|}{1.9} & 2.9 \\ \hline
% \end{tabular}
% \caption{Closed World With Rejection ROD - synROD}
% \label{tab:cw_with_rod_synrod}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|c|l|}
% \hline
%  & \multicolumn{4}{c|}{Open World} & \multicolumn{1}{l|}{} &  \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{} &  \\ \hline
% METHOD & 11 & 16 & 21 & 26 & Avg. & Harm \\ \hline
% NNO & 49.0 & 47.7 & 46.5 & 45.4 & 47.2 & 0.9 \\ \hline
%  & 48.2 & 41.7 & 41.2 & 38.9 & 42.5 & 3.5 \\ \hline
% DeepNNO & 47.0 & 34.4 & 33.2 & 30.3 & 36.2 & 7.6 \\ \hline
% DeepNNO-RDA & 45.3 & 40.1 & 38.1 & 32.5 & 39.0 & 5.2 \\ \hline
% DeepNNO-RSDA & 47.7 & 42.1 & 41.1 & 38.2 & 42.3 & 3.0 \\ \hline
% DeepNNO-rot & 47.0 & 37.7 & 35.3 & 30.6 & 37.6 & 6.2 \\ \hline
% DeepNNO-RDA-rot & 36.9 & 29.9 & 30.1 & 27.6 & 31.1 & 8.8 \\ \hline
% DeepNNO-Dropout & 40.7 & 41.9 & 44.6 & 44.9 & 43.0 & 3.7 \\ \hline
%  & 46.7 & 43.0 & 43.9 & 43.2 & 44.2 & 4.5 \\ \hline
% B-DOC & 43.4 & 40.8 & 41.9 & 42.8 & 42.2 & 5.5 \\ \hline
% B-DOC-RDA & 38.9 & 41.1 & 43.3 & 43.0 & 41.6 & 3.9 \\ \hline
% B-DOC-RSDA & 45.4 & 41.4 & 41.0 & 40.5 & 42.1 & 5.7 \\ \hline
% B-DOC-rot & 3.4 & 1.9 & 1.4 & 1.3 & 2.0 &  \\ \hline
% B-DOC-RDA-rot & \multicolumn{1}{r|}{3.6} & \multicolumn{1}{r|}{3.7} & \multicolumn{1}{r|}{2.5} & \multicolumn{1}{r|}{1.9} & 2.9 &  \\ \hline
% \end{tabular}
% \caption{OWR mean ROD - synROD}
% \label{tab:owr_rod_synrod}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
%  & \multicolumn{4}{c|}{CW without rejection} &  \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} &  \\ \hline
% METHOD & 11 & 16 & 21 & 26 & \multicolumn{1}{c|}{Avg.} \\ \hline
% DeepNNO & 21.0 & 16.3 & 14.4 & 12.0 & 15.9 \\ \hline
% DeepNNO-RSDA & 23.2 & 14.9 & 12.0 & 10.9 & 15.3 \\ \hline
% DeepNNO-RDA & 20.0 & 13.0 & 10.4 & 9.7 & 13.3 \\ \hline
% DeepNNO-rot & 19.4 & 15.1 & 14.5 & 13.0 & 15.5 \\ \hline
% DeepNNO-Dropout & 19.3 & 15.6 & 14.2 & 12.8 & 15.5 \\ \hline
% DeepNNO-RDA-rot & \multicolumn{1}{r|}{21.4} & \multicolumn{1}{r|}{13.3} & \multicolumn{1}{r|}{11.4} & \multicolumn{1}{r|}{10.5} & 14.2 \\ \hline
%  &  &  &  &  &  \\ \hline
% B-DOC & \multicolumn{1}{r|}{23.8} & \multicolumn{1}{r|}{16.0} & \multicolumn{1}{r|}{13.4} & \multicolumn{1}{r|}{12.9} & 16.5 \\ \hline
% B-DOC-RSDA & \multicolumn{1}{r|}{25.2} & \multicolumn{1}{r|}{16.7} & \multicolumn{1}{r|}{12.1} & \multicolumn{1}{r|}{11.0} & 16.3 \\ \hline
% B-DOC-rot & \multicolumn{1}{r|}{24.4} & \multicolumn{1}{r|}{17.0} & \multicolumn{1}{r|}{14.5} & \multicolumn{1}{r|}{11.9} & 17.0 \\ \hline
% B-DOC-Dropout & \multicolumn{1}{r|}{20.8} & \multicolumn{1}{r|}{16.5} & \multicolumn{1}{r|}{14.6} & \multicolumn{1}{r|}{14.0} & 16.5 \\ \hline
% B-DOC-RDA-rot & \multicolumn{1}{r|}{24.99} & \multicolumn{1}{r|}{15.80} & \multicolumn{1}{r|}{12.16} & \multicolumn{1}{r|}{9.66} & 15.7 \\ \hline
% \end{tabular}
% \caption{Closed World Without Rejection synROD - ARID}
% \label{tab:cw_without_synrod_arid}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|c|}
% \hline
%  & \multicolumn{4}{c|}{CW with rejection} & \multicolumn{1}{l|}{} \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{} \\ \hline
% METHOD & 11 & 16 & 21 & 26 & Avg. \\ \hline
% DeepNNO & 4.1 & 6.6 & 5.4 & 5.3 & 5.4 \\ \hline
% DeepNNO-RSDA & 4.1 & 5.1 & 4.3 & 3.3 & 4.2 \\ \hline
% DeepNNO-RDA & 4.0 & 4.0 & 3.6 & 4.2 & 4.0 \\ \hline
% DeepNNO-rot & 3.1 & 6.6 & 6.0 & 6.0 & 5.4 \\ \hline
% DeepNNO-Dropout & 7.3 & 9.7 & 8.8 & 8.0 & 8.4 \\ \hline
% DeepNNO-RDA-rot & \multicolumn{1}{r|}{6.4} & \multicolumn{1}{r|}{5.2} & \multicolumn{1}{r|}{4.6} & \multicolumn{1}{r|}{3.7} & 4.9 \\ \hline
%  &  &  &  &  &  \\ \hline
% B-DOC & \multicolumn{1}{r|}{2.7} & \multicolumn{1}{r|}{2.6} & \multicolumn{1}{r|}{1.7} & \multicolumn{1}{r|}{1.9} & 2.2 \\ \hline
% B-DOC-RSDA & \multicolumn{1}{r|}{3.4} & \multicolumn{1}{r|}{2.8} & \multicolumn{1}{r|}{1.8} & \multicolumn{1}{r|}{2.1} & 2.5 \\ \hline
% B-DOC-rot & \multicolumn{1}{r|}{2.4} & \multicolumn{1}{r|}{2.6} & \multicolumn{1}{r|}{1.7} & \multicolumn{1}{r|}{1.7} & 2.1 \\ \hline
% B-DOC-Dropout & \multicolumn{1}{r|}{16.1} & \multicolumn{1}{r|}{8.7} & \multicolumn{1}{r|}{7.4} & \multicolumn{1}{r|}{8.0} & 10.0 \\ \hline
% B-DOC-RDA-rot & \multicolumn{1}{r|}{3.33} & \multicolumn{1}{r|}{2.55} & \multicolumn{1}{r|}{1.61} & \multicolumn{1}{r|}{1.37} & 2.2 \\ \hline
% \end{tabular}
% \caption{Closed World With Rejection synROD - ARID}
% \label{tab:cw_wit_synrod_arid}
% \end{table}


% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|c|r|}
% \hline
%  & \multicolumn{4}{c|}{Open World} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
% METHOD & 11 & 16 & 21 & 26 & Avg. & \multicolumn{1}{l|}{Harm} \\ \hline
% DeepNNO & 43.5 & 39.9 & 40.0 & 38.3 & 40.4 & 10.0 \\ \hline
% DeepNNO-RSDA & 44.9 & 40.4 & 39.8 & 37.5 & 40.6 & 8.0 \\ \hline
% DeepNNO-RDA & 44.7 & 42.0 & 39.9 & 38.7 & 41.3 & 7.5 \\ \hline
% DeepNNO-rot & 44.2 & 37.9 & 41.0 & 38.3 & 40.4 & 10.1 \\ \hline
% DeepNNO-Dropout & 35.8 & 30.7 & 31.4 & 28.8 & 31.7 & 14.6 \\ \hline
% DeepNNO-RDA-rot & 39.1 & 38.9 & 36.9 & 38.1 & 38.3 & 9.3 \\ \hline
%  &  &  &  &  &  & \multicolumn{1}{l|}{} \\ \hline
% B-DOC & 47.7 & 47.9 & 47.4 & 47.6 & 47.7 & 4.3 \\ \hline
% B-DOC-RSDA & 47.1 & 46.8 & 46.4 & 43.7 & 46.0 & 4.9 \\ \hline
% B-DOC-rot & 48.4 & 48.1 & 48.0 & 46.9 & 47.8 & 4.1 \\ \hline
% B-DOC-Dropout & 22.0 & 27.7 & 25.6 & 26.3 & 25.4 & 16.1 \\ \hline
% B-DOC-RDA-rot & 46.9 & 47.0 & 46.2 & 45.8 & 46.5 & 4.3 \\ \hline
% \end{tabular}
% \caption{OWR mean synROD - ARID}
% \label{tab:owr_synrod_arid}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|c|}
% \hline
%  & \multicolumn{4}{c|}{CW without rejection} & \multicolumn{1}{l|}{} \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{} \\ \hline
% METHOD & 11 & 16 & 21 & 26 & Avg. \\ \hline
% DeepNNO & 33.0 & 26.2 & 21.4 & 16.8 & 24.4 \\ \hline
% DeepNNO-RSDA & 44.8 & 34.7 & 30.3 & 26.9 & 34.2 \\ \hline
% DeepNNO-RDA & 39.8 & 33.9 & 28.2 & 24.9 & 31.7 \\ \hline
% DeepNNO-rot & 35.3 & 29.0 & 23.7 & 19.4 & 26.8 \\ \hline
% DeepNNO-Dropout & 34.5 & 27.8 & 24.1 & 17.4 & 25.9 \\ \hline
% DeepNNO-RDA-rot & \multicolumn{1}{r|}{43.0} & \multicolumn{1}{r|}{35.4} & \multicolumn{1}{r|}{31.0} & \multicolumn{1}{r|}{26.9} & 34.1 \\ \hline
%  &  &  &  &  &  \\ \hline
% B-DOC & \multicolumn{1}{r|}{36.2} & \multicolumn{1}{r|}{30.5} & \multicolumn{1}{r|}{23.4} & \multicolumn{1}{r|}{20.1} & 27.6 \\ \hline
% B-DOC-RSDA & \multicolumn{1}{r|}{49.7} & \multicolumn{1}{r|}{40.3} & \multicolumn{1}{r|}{34.2} & \multicolumn{1}{r|}{27.5} & 37.9 \\ \hline
% B-DOC-rot & \multicolumn{1}{r|}{37.9} & \multicolumn{1}{r|}{35.0} & \multicolumn{1}{r|}{26.6} & \multicolumn{1}{r|}{19.3} & 29.7 \\ \hline
% B-DOC-Dropout & \multicolumn{1}{r|}{36.7} & \multicolumn{1}{r|}{28.6} & \multicolumn{1}{r|}{22.8} & \multicolumn{1}{r|}{18.9} & 26.7 \\ \hline
% B-DOC-RDA-rot & \multicolumn{1}{r|}{49.51} & \multicolumn{1}{r|}{40.22} & \multicolumn{1}{r|}{32.51} & \multicolumn{1}{r|}{21.25} & 35.9 \\ \hline
% \end{tabular}
% \caption{Closed World Without Rejection synROD - ROD}
% \label{tab:cw_without_synrod_rod}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|c|}
% \hline
%  & \multicolumn{4}{c|}{CW with rejection} & \multicolumn{1}{l|}{} \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{} \\ \hline
% METHOD & 11 & 16 & 21 & 26 & Avg. \\ \hline
% DeepNNO & 13.0 & 10.9 & 8.5 & 6.1 & 9.6 \\ \hline
% DeepNNO-RSDA & 17.8 & 15.4 & 12.1 & 10.6 & 14.0 \\ \hline
% DeepNNO-RDA & 13.3 & 13.1 & 11.4 & 10.6 & 12.1 \\ \hline
% DeepNNO-rot & 12.9 & 13.0 & 9.6 & 6.4 & 10.5 \\ \hline
% DeepNNO-Dropout & 21.8 & 18.5 & 15.9 & 11.9 & 17.0 \\ \hline
% DeepNNO-RDA-rot & \multicolumn{1}{r|}{20.1} & \multicolumn{1}{r|}{16.0} & \multicolumn{1}{r|}{13.5} & \multicolumn{1}{r|}{12.1} & 15.4 \\ \hline
%  &  &  &  &  &  \\ \hline
% B-DOC & \multicolumn{1}{r|}{10.0} & \multicolumn{1}{r|}{5.7} & \multicolumn{1}{r|}{2.9} & \multicolumn{1}{r|}{2.3} & 5.2 \\ \hline
% B-DOC-RSDA & \multicolumn{1}{r|}{19.4} & \multicolumn{1}{r|}{11.2} & \multicolumn{1}{r|}{6.3} & \multicolumn{1}{r|}{6.2} & 10.8 \\ \hline
% B-DOC-rot & \multicolumn{1}{r|}{7.7} & \multicolumn{1}{r|}{6.4} & \multicolumn{1}{r|}{3.3} & \multicolumn{1}{r|}{3.2} & 5.1 \\ \hline
% B-DOC-Dropout & \multicolumn{1}{r|}{26.6} & \multicolumn{1}{r|}{18.3} & \multicolumn{1}{r|}{14.9} & \multicolumn{1}{r|}{12.3} & 18.0 \\ \hline
% B-DOC-RDA-rot & \multicolumn{1}{r|}{17.07} & \multicolumn{1}{r|}{11.57} & \multicolumn{1}{r|}{5.89} & \multicolumn{1}{r|}{4.13} & 9.7 \\ \hline
% \end{tabular}
% \caption{Closed World With Rejection synROD - ROD}
% \label{tab:cw_wit_synrod_rod}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|c|r|}
% \hline
%  & \multicolumn{4}{c|}{Open World} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
% METHOD & 11 & 16 & 21 & 26 & Avg. & \multicolumn{1}{l|}{Harm} \\ \hline
% DeepNNO & 44.5 & 43.9 & 42.0 & 37.9 & 42.0 & 17.0 \\ \hline
% DeepNNO-RSDA & 48.2 & 46.1 & 43.0 & 39.4 & 44.2 & 23.5 \\ \hline
% DeepNNO-RDA & 46.3 & 46.1 & 42.1 & 41.1 & 43.9 & 20.9 \\ \hline
% DeepNNO-rot & 46.7 & 43.6 & 43.3 & 37.9 & 42.9 & 18.4 \\ \hline
% DeepNNO-Dropout & 38.0 & 34.3 & 32.4 & 27.8 & 33.1 & 25.3 \\ \hline
% DeepNNO-RDA-rot & 44.4 & 44.5 & 40.8 & 40.1 & 42.4 & 25.2 \\ \hline
%  &  &  &  &  &  & \multicolumn{1}{l|}{} \\ \hline
% B-DOC & 47.6 & 48.1 & 47.5 & 45.7 & 47.2 & 9.9 \\ \hline
% B-DOC-RSDA & 50.2 & 48.9 & 46.7 & 44.4 & 47.6 & 19.1 \\ \hline
% B-DOC-rot & 48.5 & 49.4 & 48.4 & 44.3 & 47.6 & 9.7 \\ \hline
% B-DOC-Dropout & 23.2 & 28.0 & 26.2 & 23.6 & 25.2 & 23.2 \\ \hline
% B-DOC-RDA-rot & 47.3 & 48.7 & 46.4 & 45.1 & 46.9 & 17.3 \\ \hline
% \end{tabular}
% \caption{OWR mean synROD - ROD}
% \label{tab:owr_synrod_rod}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|c|}
% \hline
%  & \multicolumn{4}{c|}{CW without rejection} & \multicolumn{1}{l|}{} \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{} \\ \hline
% METHOD & 11 & 16 & 21 & 26 & Avg. \\ \hline
% DeepNNO & 54.0 & 45.4 & 43.8 & 41.1 & 46.1 \\ \hline
% DeepNNO-RSDA & 61.1 & 52.7 & 48.4 & 44.1 & 51.6 \\ \hline
% DeepNNO-RDA & 59.5 & 51.4 & 47.9 & 43.4 & 50.5 \\ \hline
% DeepNNO-rot & 54.5 & 46.8 & 47.4 & 43.5 & 48.1 \\ \hline
% DeepNNO-Dropout & 53.8 & 45.1 & 43.4 & 40.9 & 45.8 \\ \hline
% DeepNNO-RDA-rot & \multicolumn{1}{r|}{62.2} & \multicolumn{1}{r|}{54.1} & \multicolumn{1}{r|}{50.0} & \multicolumn{1}{r|}{45.9} & 53.1 \\ \hline
%  &  &  &  &  &  \\ \hline
% B-DOC & \multicolumn{1}{r|}{55.5} & \multicolumn{1}{r|}{46.7} & \multicolumn{1}{r|}{45.9} & \multicolumn{1}{r|}{42.5} & 47.6 \\ \hline
% B-DOC-RSDA & \multicolumn{1}{r|}{65.1} & \multicolumn{1}{r|}{56.8} & \multicolumn{1}{r|}{52.8} & \multicolumn{1}{r|}{48.0} & 55.7 \\ \hline
% B-DOC-rot & \multicolumn{1}{r|}{55.6} & \multicolumn{1}{r|}{48.3} & \multicolumn{1}{r|}{47.5} & \multicolumn{1}{r|}{40.0} & 47.9 \\ \hline
% B-DOC-Dropout & \multicolumn{1}{r|}{54.0} & \multicolumn{1}{r|}{45.2} & \multicolumn{1}{r|}{42.3} & \multicolumn{1}{r|}{39.1} & 45.1 \\ \hline
% B-DOC-RDA-rot & \multicolumn{1}{r|}{65.1} & \multicolumn{1}{r|}{57.7} & \multicolumn{1}{r|}{52.2} & \multicolumn{1}{r|}{39.3} & 53.6 \\ \hline
% \end{tabular}
% \caption{Closed World Without Rejection synROD - synROD}
% \label{tab:cw_without_synrod_synrod}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|c|}
% \hline
%  & \multicolumn{4}{c|}{CW with rejection} & \multicolumn{1}{l|}{} \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{} \\ \hline
% METHOD & 11 & 16 & 21 & 26 & Avg. \\ \hline
% DeepNNO & 32.7 & 27.3 & 27.6 & 26.0 & 28.4 \\ \hline
% DeepNNO-RSDA & 34.1 & 32.3 & 31.7 & 26.3 & 31.1 \\ \hline
% DeepNNO-RDA & 34.8 & 30.2 & 29.5 & 26.9 & 30.4 \\ \hline
% DeepNNO-rot & 34.4 & 29.7 & 30.0 & 27.6 & 30.4 \\ \hline
% DeepNNO-Dropout & 40.3 & 36.3 & 35.2 & 32.9 & 36.2 \\ \hline
% DeepNNO-RDA-rot & \multicolumn{1}{r|}{41.2} & \multicolumn{1}{r|}{33.7} & \multicolumn{1}{r|}{32.4} & \multicolumn{1}{r|}{28.4} & 33.9 \\ \hline
%  &  &  &  &  &  \\ \hline
% B-DOC & \multicolumn{1}{r|}{29.7} & \multicolumn{1}{r|}{20.8} & \multicolumn{1}{r|}{18.9} & \multicolumn{1}{r|}{14.4} & 20.9 \\ \hline
% B-DOC-RSDA & \multicolumn{1}{r|}{36.8} & \multicolumn{1}{r|}{28.1} & \multicolumn{1}{r|}{23.8} & \multicolumn{1}{r|}{19.6} & 27.1 \\ \hline
% B-DOC-rot & \multicolumn{1}{r|}{28.7} & \multicolumn{1}{r|}{20.4} & \multicolumn{1}{r|}{18.9} & \multicolumn{1}{r|}{13.4} & 20.4 \\ \hline
% B-DOC-Dropout & \multicolumn{1}{r|}{45.0} & \multicolumn{1}{r|}{35.1} & \multicolumn{1}{r|}{32.5} & \multicolumn{1}{r|}{26.8} & 34.8 \\ \hline
% B-DOC-RDA-rot & \multicolumn{1}{r|}{38.7} & \multicolumn{1}{r|}{27.4} & \multicolumn{1}{r|}{21.8} & \multicolumn{1}{r|}{15.1} & 25.7 \\ \hline
% \end{tabular}
% \caption{Closed World With Rejection synROD - synROD}
% \label{tab:cw_with_synrod_synrod}
% \end{table}

% \begin{table}[t]
% \centering
% \begin{tabular}{|l|l|l|l|l|c|r|}
% \hline
%  & \multicolumn{4}{c|}{Open World} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
%  & \multicolumn{4}{c|}{KNOWN CLASSES} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
% METHOD & 11 & 16 & 21 & 26 & Avg. & \multicolumn{1}{l|}{Harm} \\ \hline
% DeepNNO & 51.9 & 49.0 & 49.0 & 48.0 & 49.5 & 40.5 \\ \hline
% DeepNNO-RSDA & 52.3 & 51.1 & 49.3 & 46.9 & 49.9 & 42.8 \\ \hline
% DeepNNO-RDA & 51.4 & 50.2 & 48.4 & 45.8 & 48.9 & 41.9 \\ \hline
% DeepNNO-rot & 54.7 & 49.6 & 50.1 & 49.8 & 51.0 & 42.7 \\ \hline
% DeepNNO-Dropout & 43.4 & 38.6 & 38.3 & 35.6 & 39.0 & 38.8 \\ \hline
% DeepNNO-RDA-rot & 51.0 & 49.5 & 48.4 & 46.0 & 48.8 & 44.2 \\ \hline
%  &  &  &  &  &  & \multicolumn{1}{l|}{} \\ \hline
% B-DOC & 53.7 & 53.0 & 53.5 & 51.4 & 52.9 & 33.6 \\ \hline
% B-DOC-RSDA & 55.1 & 53.8 & 52.7 & 49.7 & 52.8 & 40.3 \\ \hline
% B-DOC-rot & 54.8 & 53.0 & 53.7 & 47.9 & 52.3 & 32.8 \\ \hline
% B-DOC-Dropout & 30.0 & 29.1 & 29.3 & 27.5 & 29.0 & 27.8 \\ \hline
% B-DOC-RDA-rot & 54.3 & 52.9 & 51.7 & 47.1 & 51.5 & 38.6 \\ \hline
% \end{tabular}
% \caption{OWR mean synROD - synROD}
% \label{tab:owr_without_synrod_synrod}
% \end{table}
